On the Privacy-Robustness-Utility Trilemma in Distributed Learning

The ubiquity of distributed machine learning (ML) in sensitive public domain applications calls for algorithms that protect data privacy, while being robust to faults and adversarial behaviors. Although privacy and robustness have been extensively studied independently in distributed ML, their synthesis remains poorly understood. We present the first tight analysis of the error incurred by any algorithm ensuring robustness against a fraction of adversarial machines, as well as differential privacy (DP) for honest machines' data against any other curious entity. Our analysis exhibits a fundamental trade-off between privacy, robustness, and utility. To prove our lower bound, we consider the case of mean estimation, subject to distributed DP and robustness constraints, and devise reductions to centralized estimation of one-way marginals. We prove our matching upper bound by presenting a new distributed ML algorithm using a high-dimensional robust aggregation rule. The latter amortizes the dependence on the dimension in the error (caused by adversarial workers and DP), while being agnostic to the statistical properties of the data.

==> experiments.tex <==
\section{Experimental Evaluation}
\label{sec:exp}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.5\textwidth]{plots/svm-phishing_empire_f=3_privacy=7.5_lr=2_clip=0.01.pdf}%
    \includegraphics[width=0.5\textwidth]{plots/svm-phishing_labelflipping_f=3_privacy=7.5_lr=2_clip=0.01.pdf}\\%
    \caption{Experiments on Phishing with $f = 3$ adversarial workers among $n = 7$ workers, with $\beta = 0.99$. The adversarial workers execute the FOE (\textit{left}) and LF (\textit{right}) attacks. Privacy budget after $T = 400$ steps is $(\epsilon, \delta) = (0.07, 10^{-4})$.}
\label{fig:plots_phishing_main}
\end{figure*}
